Prospects on the search for invisible Higgs decays in the ZH channel at the LHC and HL-LHC: A Snowmass White Paper

We show prospects on a search for invisible decays of a Higgs boson at the Large Hadron Collider (LHC) and High Luminosity LHC (HL-LHC). This search is performed on a Higgs boson produced in association with a Z boson. We expect that the branching ratio of 17-22% (6-14%) could be excluded at 95% confidence level with 300 fb^{-1} (3000 fb^{-1}) of data at sqrt(s)=14 TeV. The range indicates different assumptions on the control of systematic uncertainties. Interpretations with Higgs-portal dark matter models are also considered.

==> biblio.tex <==

\begin{thebibliography}{55}
%
%\cite{Arnold:2012xn}
\bibitem{Arnold:2012xn} 
  K.~Arnold, J.~Bellm, G.~Bozzi, F.~Campanario, C.~Englert, B.~Feigl, J.~Frank and T.~Figy {\it et al.},
  %``Release Note -- Vbfnlo-2.6.0,''
  arXiv:1207.4975 [hep-ph].
  %%CITATION = ARXIV:1207.4975;%%

%\cite{Bozzi:2012mh}
\bibitem{Bozzi:2012mh} 
  G.~Bozzi, F.~Campanario, C.~NEnglert, M.~Rauch, M.~Spannoswky and D.~Zeppenfeld,
  %``Precision Multiboson Phenomenology,''
  arXiv:1205.2506 [hep-ph].
  %%CITATION = ARXIV:1205.2506;%%

%\cite{Kilian:2007gr}
\bibitem{Kilian:2007gr} 
  W.~Kilian, T.~Ohl and J.~Reuter,
  %``WHIZARD: Simulating Multi-Particle Processes at LHC and ILC,''
  Eur.\ Phys.\ J.\ C {\bf 71}, 1742 (2011)
  [arXiv:0708.4233 [hep-ph]].
  %%CITATION = ARXIV:0708.4233;%%

%\cite{Christensen:2010wz}
\bibitem{Christensen:2010wz} 
  N.~D.~Christensen, C.~Duhr, B.~Fuks, J.~Reuter and C.~Speckner,
  %``Introducing an interface between WHIZARD and FeynRules,''
  Eur.\ Phys.\ J.\ C {\bf 72}, 1990 (2012)
  [arXiv:1010.3251 [hep-ph]].
  %%CITATION = ARXIV:1010.3251;%%

%\cite{Degrande:2012wf}
\bibitem{Degrande:2012wf} 
  C.~Degrande, N.~Greiner, W.~Kilian, O.~Mattelaer, H.~Mebane, T.~Stelzer, S.~Willenbrock and C.~Zhang,
  %``Effective Field Theory: A Modern Approach to Anomalous Couplings,''
  arXiv:1205.4231 [hep-ph].
  %%CITATION = ARXIV:1205.4231;%%

%\cite{Corbett:2013pja}
\bibitem{Corbett:2013pja} 
  T.~Corbett, O.~J.~P.~Eboli, J.~Gonzalez-Fraile and M.~C.~Gonzalez-Garcia,
  %``Determining Triple Gauge Boson Couplings from Higgs Data,''
  arXiv:1304.1151 [hep-ph].
  %%CITATION = ARXIV:1304.1151;%%
  %2 citations counted in INSPIRE as of 06 Jun 2013

%\cite{Hagiwara:1993ck}
\bibitem{Hagiwara:1993ck} 
  K.~Hagiwara, S.~Ishihara, R.~Szalapski and D.~Zeppenfeld,
  %``Low-energy effects of new interactions in the electroweak boson sector,''
  Phys.\ Rev.\ D {\bf 48}, 2182 (1993).
  %%CITATION = PHRVA,D48,2182;%%


%\cite{Hagiwara:1986vm}
\bibitem{Hagiwara:1986vm} 
  K.~Hagiwara, R.~D.~Peccei, D.~Zeppenfeld and K.~Hikasa,
  %``Probing the Weak Boson Sector in e+ e- ---> W+ W-,''
  Nucl.\ Phys.\ B {\bf 282}, 253 (1987).
  %%CITATION = NUPHA,B282,253;%%
  
  %add by CD below this  point
  
  \bibitem{Grzadkowski:2010es} 
  B.~Grzadkowski, M.~Iskrzynski, M.~Misiak and J.~Rosiek,
  %``Dimension-Six Terms in the Standard Model Lagrangian,''
  JHEP {\bf 1010}, 085 (2010)
  [arXiv:1008.4884 [hep-ph]].
  %%CITATION = ARXIV:1008.4884;%%
  %76 citations counted in INSPIRE as of 19 Jun 2013
  
\bibitem{Wudka:1994ny} 
  J.~Wudka,
  %``Electroweak effective Lagrangians,''
  Int.\ J.\ Mod.\ Phys.\ A {\bf 9}, 2301 (1994)
  [hep-ph/9406205].
  %%CITATION = HEP-PH/9406205;%%
  %100 citations counted in INSPIRE as of 19 Jun 2013

\bibitem{Eboli:2006wa} O.~J.~P.~Eboli, M.~C.~Gonzalez-Garcia and
  J.~K.~Mizukoshi, ``$p p \to j j e^\pm \mu^\mp \nu \nu$ and $j j
  e^\pm \mu^\mp \nu \nu$ at $\cal{ O}( \alpha_{em}^6)$ and ${\cal
    O}(\alpha_{em}^4 \alpha_s^2)$ for the study of the quartic
  electroweak gauge boson vertex at CERN LHC,'' Phys.\ Rev.\ D {\bf
    74}, 073005 (2006) [hep-ph/0606118].
  %%CITATION = HEP-PH/0606118;%%

%\cite{Arzt:1994gp}
\bibitem{Arzt:1994gp} 
  C.~Arzt, M.~B.~Einhorn and J.~Wudka,
  %``Patterns of deviation from the standard model,''
  Nucl.\ Phys.\ B {\bf 433}, 41 (1995)
  [hep-ph/9405214].
  %%CITATION = HEP-PH/9405214;%%
  %151 citations counted in INSPIRE as of 28 Jun 2013

\bibitem{quarticATlep} See for instance, and references therein,
http://pdg.lbl.gov/2010/reviews/rpp2010-rev-wz-quartic-couplings.pdf.



\end{thebibliography}

